Convergences and Divergences between Automatic Assessment and Human Evaluation: Insights from Comparing ChatGPT-Generated Translation and Neural Machine Translation

Large language models have demonstrated parallel and even superior translation performance compared to neural machine translation (NMT) systems. However, existing comparative studies between them mainly rely on automated metrics, raising questions into the feasibility of these metrics and their alignment with human judgment. The present study investigates the convergences and divergences between automated metrics and human evaluation in assessing the quality of machine translation from ChatGPT and three NMT systems. To perform automatic assessment, four automated metrics are employed, while human evaluation incorporates the DQF-MQM error typology and six rubrics. Notably, automatic assessment and human evaluation converge in measuring formal fidelity (e.g., error rates), but diverge when evaluating semantic and pragmatic fidelity, with automated metrics failing to capture the improvement of ChatGPT's translation brought by prompt engineering. These results underscore the indispensable role of human judgment in evaluating the performance of advanced translation tools at the current stage.

==> sec1-introduction.tex <==
\section{Introduction}\label{sec:intro}
Against the backdrop of translation automation and the advances in translation technology, neural machine translation (hereafter NMT) has been widely investigated under both academic and professional scenarios~\citep{Gaspari2015}. % Based on the encoder-decoder neural network architecture, NMT has greatly reduced the number of grammatical mistakes as witnessed in older statistical MT systems, and possesses the ability to capture long-range contextual information, and learn domain-specific linguistic patterns from corpus data~\citep{Cho2014}. 
Scholars have discussed its applications across different domains, and found it to fare well in both non-literary and literary texts, demonstrating satisfying quality and even creativity to some degree~\citep{Hu-Li2023}. 

In recent years, the emergence of large language models (LLMs) has further revolutionized the relationship between translation technologies and translators, and has opened up new possibilities for interactive translation using customized prompts, making proficiency in using AI tools an integral part of digital literacy~\citep{Godwin-Jones2022}. Among them, ChatGPT, an AI-powered LLM designed and trained by OpenAI1, has demonstrated remarkable capabilities in a wide range of tasks, including translation among others~\citep{Hendy2023,Lai2023,2020MMLU,2022BIG-Bench,Zhao2023,2023codesurvey}. Recent studies have shown that ChatGPT is in par with or surpasses mainstream NMT engines in translating news, user comments, conversation, social media posts, and scientific texts~\citep{Jiao2023,Hendy2023,Wang2023,Peng2023,Lu2023,Chen2023,He2023,Kocmi2023,2023Comparison}.

The earlier explorations focusing on translation quality assessment (TQA) of machine translation have demonstrated the promising role of ChatGPT in generating quality translations. However, most of these studies are conducted on huge translation corpora, and the scholars mostly rely on automated metrics and scarcely resort to human evaluation, which only serves as a complement to automated metrics. 

\begin{figure*}
    \centering
    \includegraphics[width=0.325\textwidth]{figures/error-penalty.png}
    \includegraphics[width=0.33\textwidth]{figures/error-severity.jpg}
    \includegraphics[width=0.33\textwidth]{figures/correlation.png}
    \caption{Total error penalty (left) and proportion of error severity (middle) assigned by human annotators to different translations. Right: correlation coefficients between human evaluation and automated metrics.}
    \label{fig:human-error-correlation}
\end{figure*}


As NMT systems and LLMs keep making improvements, these measures may fail to fully capture the quality of machine translation. In particular, we have limited understanding of what aspects or dimensions other than content overlap can really define high-quality machine translations and distinguish them from those low-quality ones. There is a lack of metrics that are capable of measuring translation quality as humans do, who pay attention to dimensions such as intended audience, cultural sensitivity, adherence to translation norms, textual coherence, and practicality. Also, previous research is often conducted on extensive, publicly available datasets that are crawled from the internet and encompass diverse domains\footnote{In this work, the terms ``domain'' and ``'register'' are used interchangeably. The former is preferred by the AI community. The later is preferred by linguistics literature.}, genres, and text types. There seems to be a scarcity of high-quality, domain-specific parallel corpora that would enable more focused and specialized quality assessment in machine translation. 
% Another issue is that quality is often represented solely by accuracy, whether measured as the alignment with human reference, i.e. reference-based metrics such as BLEU~\citep{2002BLEU}, chfF~\citep{2015chrF,2017chrF++}, BERTScore~\citep{2019BERTScore}, and BLEURT~\citep{2020BLEURT}, or the extent to which the translation accurately reflects the semantic meaning of the source text, i.e. reference-free metrics such as YiSi-2~\citep{2018YiSi}, SentSim~\citep{2021SentSim}, and XBERTScore~\citep{2021XBERTScore}. However, as NMT systems and LLMs keep making improvements, these measures may fail to fully capture the quality of machine translation. In particular, we have limited understanding of what aspects or dimensions other than accuracy can really define high-quality machine translations and distinguish them from those low-quality ones. There is a lack of metrics that do not rely solely on computable aspects, but are capable of measuring translation quality as humans do, which pay attention to dimensions such as cultural sensitivity, adherence to translation norms, textual coherence, and practicality. Also, previous research is often conducted on extensive, publicly available datasets that are crawled from the internet and encompass diverse domains\footnote{In this work, the terms ``domain'' and ``'register'' are used interchangeably. The former is preferred by the AI community. The later is preferred by linguistics literature.}, genres, and text types. There seems to be a scarcity of high-quality, domain-specific parallel corpora that would enable more focused and specialized quality assessment in machine translation. 

Thus, we focus on a specific domain, and construct our major research questions as follows:

\begin{enumerate}
    \item How well do NMT systems and ChatGPT perform under automated assessment?
    \item How well do NMT systems and ChatGPT perform under human evaluation? 
    \item To what degree do automated metrics align with human evaluation?
\end{enumerate}

 
Essentially, RQ1 and RQ2 aim to provide a well-rounded assessment of translations from NMT systems and ChatGPT using both automated metrics and human evaluation. Based on RQ1 and RQ2, RQ3 taps into the inter-correlation between automated metrics and human scores. For RQ1 and RQ2, we find that ChatGPT excels under human evaluation and semantic-aware automatic evaluation (see Figure~\ref{fig:human-error-correlation} and Table~\ref{tab:results-auto}). For RQ3, we find that the two methods may exhibit divergences when approaching machine-translated texts, contrary to \citet{2023Lu-Han}'s findings that automated metrics can show moderate to strong correlations with human-assigned scores in assessing interpreting outputs, possibly due to the inherent differences between interpreting and translation.
